Calculating modules in contextual logic program refinement

The refinement calculus for logic programs is a framework for deriving logic programs from specifications. It is based on a wide-spectrum language that can express both specifications and code, and a refinement relation that models the notion of correct implementation. In this paper we extend and generalise earlier work on contextual refinement. Contextual refinement simplifies the refinement process by abstractly capturing the context of a subcomponent of a program, which typically includes information about the values of the free variables. This paper also extends and generalises module refinement. A module is a collection of procedures that operate on a common data type; module refinement between a specification module A and an implementation module C allows calls to the procedures of A to be systematically replaced with calls to the corresponding procedures of C. Based on the conditions for module refinement, we present a method for calculating an implementation module from a specification module. Both contextual and module refinement within the refinement calculus have been generalised from earlier work and the results are presented in a unified framework.

==> semantics.tex <==
\section{Semantics}
\label{semantics}

We present a simpler semantics for the wide-spectrum language than the 
state-based semantics presented in \cite{reflp:01}.  
As shown in \cite{Thesis}, the predicate and state-based
semantics have a straightforward
relationship for non-parameterised commands.
This allows us to both use and
prove laws for the basic constructs in our language using the more
intuitive predicate semantics.
This is particularly useful for defining contexts in which
refinement takes place, as the predicates $ok$ and $ef$
may be used to succinctly express the context provided by a program.
We only use two procedure-based rules in this paper, both of which
have been proven correct in \cite{Thesis}.

\subsection{Predicates}
A {\em binding\/} maps every variable to a value.
Each binding corresponds to a single ground answer to a Prolog-like query.
A {\em predicate\/} is a mapping from bindings to booleans.
%\begin{zed}
  %Predicate == Bnd \fun \bool
%\end{zed}
A predicate is therefore true or false when provided with a binding for its
free variables.
This definition is similar to the predicates of
Back and von Wright \cite{Back:98}.
We allow the usual first-order formulas as predicates,
and we
also assume a rich set of predicate primitives, such as those provided by the Z
specification notation \cite{Spivey:92}.

At times we need to distinguish between predicate implication, $\imp$, and
meta-level implication (entailment), $\entails$.
The boolean $A \entails B$, where $A$ and $B$ are $Predicates$,
is $true$ when, for all bindings $b$,
if $A.b$ holds then $B.b$ holds.
We may define $\entails$, and the corresponding
equivalence operator, as follows.
\[
    A \entails B == (\all b:Bnd @ A.b \imp B.b) \\
    A \equiv B == (\all b:Bnd @ A.b \iff B.b) 
\]


%\subsection{Terms}
%\label{def-term}
A {\em term\/} is a variable or a functor with a (possibly empty)
sequence of terms (the arguments).

\COMMENT{
\begin{syntax}
  Term ::= varT \ldata Var \rdata | funT \ldata Fun \cross \seq Term \rdata
\end{syntax}
For any variable $v$, $varT(v)$ is a term,
and
if $f$ is a functor and $ts$ is a sequence of
terms, then $funT(f,ts)$ is a term.
We restrict our universe to only include finite terms
(allowing infinite terms in the universe is discussed in
\cite{semanticsTR:00}).
}



\subsection{Effect/ok}

To define the semantics of the language, we consider the effect
of a program if assumptions are ignored, and the conditions under which
programs are guaranteed not to abort.

\paragraph{Program effect}
We define a function $ef$, which gives the
effect of a program as a characteristic predicate of the results computed
by the program, ignoring assumptions.  The effect function for the basic
constructs in our language is detailed in Fig.~\ref{figure-ok-ef}(a).
The effect of a specification is its characteristic predicate, while an
assumption has no effect.  The effect of the wide-spectrum operators and
quantifiers matches their logical counterparts, with sequential conjunction
having the same effect as parallel conjunction.



\paragraph{No abort}
We define a function $ok$, which
defines the circumstances under which a program is
guaranteed not to abort.  The details of $ok$ for basic constructs
are given in Fig.~\ref{figure-ok-ef}(b).  A specification never aborts; an
assumption aborts when its predicate is false; a parallel conjunction or a
disjunction aborts if either branch aborts.  The sequential conjunction $(S,T)$
aborts either if $S$ aborts, or if $S$ succeeds and $T$ aborts (if $S$ fails,
$T$ is not executed at all).  Both types of quantification must not abort for
any instantiation of the quantified variable.
The expression $\replace{S}{V}{K}$ represents the command $S$ with all
occurrences of free variable $V$ replaced with term $K$.

\COMMENT{
The effect of a program is therefore simply the predicate described by
the specification statements. 
Most of the manipulation of a program occurs at this level,
only appealing to assumptions for contextual information.

The $ok$ function extracts the assumptions that a command must make in
order not to abort.
It therefore acts similarly to a precondition, which we may use as
context.
}

\begin{figure}[thbp]
\begin{center}
\subfigure[The effect of program constructs]{
\begin{tabular}{rcl}
  $ef.\Spec{P}                       $&$ == $&$ P $\\
  $ef.\{ A \}                    $&$ == $&$ true $\\
  %% $ef.(\lnot S)                 $&$ == $&$ \lnot ef.S $\\
  $ef.(S \lor T)                 $&$ == $&$ ef.S \lor ef.T $\\
  $ef.(S \land T)                $&$ == $&$ ef.S \land ef.T $\\
  $ef.(S,T)                      $&$ == $&$ ef.S \land ef.T $\\
  $ef.(\exists V @ S)           $&$ == $&$ (\exists V @ ef.S) $\\
  $ef.(\forall V @ S)            $&$ == $&$ (\forall V @ ef.S) $\\
  $ef.pc(K)                     $&$  == $&$ ef.( \replace{S}{F}{K} )$
\end{tabular}
}
\subfigure[Non aborting conditions of program con\-structs]{
\begin{tabular}{rcl}
  $ok.\Spec{P}                   $&$ == $&$ true $\\
  $ok.\{ A \}                $&$ == $&$ A $\\
  %% $ok.(\lnot S)                 $&$ == $&$ ok.S $\\
  $ok.(S \lor T)             $&$ == $&$ ok.S \land ok.T $\\
  $ok.(S \land T)            $&$ == $&$ ok.S \land ok.T $\\
  $ok.(S,T)                  $&$ == $&$ ok.S \land (ef.S \implies ok.T) $\\
  $ok.(\exists V @ S)        $&$ == $&$ (\forall V @ ok.S)$\\
  $ok.(\forall V @ S)        $&$ == $&$ (\forall V @ ok.S) $\\
  $ok.pc(K)                  $&$ == $&$ ok.(\replace{S}{F}{K}) $
\end{tabular}
}
\end{center}
\vskip -4mm
\caption{Predicate semantics of basic commands}
\label{figure-ok-ef}
\end{figure}


%The original semantics also included a function $def$.   
In \cite{reflp:01},
a check on the function $def$ was also included on the
predicates in the $ok$ of specifications and assumptions.
An expression $def.A$,
where $A$ is a predicate, is true if $A$ is defined, that is, does not include
expressions such as division by zero.
%A check on $def$ was included on the
%predicates in the $ok$ of specifications and assumptions.  
To avoid this complication,
in examples that include possible undefinedness
we have included assumptions so
that the $def$ predicate would be satisfied.
We therefore avoid the explicit inclusion of $def$ in this paper.
%For simplicity we
%have not included $def$ in this paper; 
%we assume that all predicates are defined for all bindings.
%However,
%In examples that include possible undefinedness, such as division by zero, 
%we have included assumptions so
%that the $def$ predicate would be satisfied.
%The inclusion of $def$ at a later date will not invalidate any of the
%examples.


\subsection{Refinement}

Refinement between programs is defined by reducing the circumstances
under which abortion is possible --- that is, by weakening $ok$ ---
while maintaining the effect in those cases where abortion is not
possible.  Our definition is thus:
{\Defn Refinement \label{pred:refsto}}
\[
    S \refsto T \hskip 2mm == \hskip 2mm 
        ok.S \entails (ok.T \land (ef.S \iff ef.T))
        %%(\all b:Bnd @ (ok.S \imp (ok.T \land (ef.S \iff ef.T))).b)
\]

This definition of refinement does not allow the reduction of
nondeter\-minism that imperative refinement allows; in logic
programming we are interested in
$all$ possible solutions, and hence any
refinement must also return all of those solutions.
%In \cite{Hemer:nondet} a semantics for demonic nondeterminism in the
%logic programming refinement calculus is described, where a program
%may choose between sets of answers. 

Program equivalence ($\refeq$) is defined as refinement in both
directions.
{\Defn Refinement equivalence \label{pred:refeq}}
\[
    S \refeq T \hskip 2mm == \hskip 2mm 
        (S \refsto T) \land (T \refsto S)
    %S \refeq T == (\all b:Bnd @ (S \refsto T).b \land (T \refsto S).b)
\]
Typically we use the expanded version of this definition.
\begin{equation}
\label{pred:refeq:exp}
    S \refeq T \iff (ok.S \equiv ok.T) \land (ok.S \entails (ef.S \iff ef.T))
\end{equation}

\subsection{Refinement laws}
\label{pred:reftlaws}

To illustrate the refinement semantics, we show some refinement laws that have
been proven correct with respect to the above semantics
(see \cite{Thesis}).
%Throughout the paper we also use many other refinement laws,
%all of which are presented in \refappendix{ax}.

\reflaw{weaken:ass} allows an assumption to be weakened.
This corresponds to strengthening of the
conditions under which the program can abort.
{\ReftLaw Weaken assumption \label{weaken:ass}}
\[
    \Rule{A \entails B}
    {\Ass{A} \refsto \Ass{B}}
\]

\reflaw{remove:ass} allows an assumption to be removed from a program at any
time.
{\ReftLaw Remove assumption \label{remove:ass}}
\[
    \Ass{A}, S \refsto S
\]

\reflaw{equiv:specs:rc} allows
the characteristic predicate of a specification to be replaced with an
equivalent predicate.  This corresponds to keeping the effect of a program
equivalent.
{\ReftLaw Equivalent specifications \label{equiv:specs:rc}}
\[
    \Rule{P \equiv Q}
        {\Spec{P} \refeq \Spec{Q}}
\]

\reflaw{ctx:ass:spec:refsto:rc}
demonstrates the effect of contextual refinement.  It is similar to
\reflaw{equiv:specs:rc}, however we may use the assumption $A$ in discharging
the proof obligation $P \iff Q$.  We discuss contextual refinement in more
detail in \refsect{context}. 
{\ReftLaw Assumption in context \label{ctx:ass:spec:refsto:rc}}
\[  
    \Rule{A \entails (P \iff Q)}
        {\Ass{A}, \Spec{P} \refsto \Ass{A}, \Spec{Q}}
\]  

\reflaw{lift:disj} allows predicate disjunction to be lifted to program
disjunction when the disjunction appears inside a specification.  Predicate
conjunction and quantification may also be lifted to their program counterparts
when they appear inside specifications 
%(lifting laws are 
%presented in \refappendix{lifting}).
{\ReftLaw Lift disjunction \label{lift:disj}}
\[  
    \Spec{P \lor Q} \refeq \Spec{P} \lor \Spec{Q}
\]

\reflaw{mono:para}
is an example of a monotonicity law.  In general, a monotonicity law
states that the refinement of a component of a program refines the entire
program.
In this case,
that $S$ refines to $S'$ and $T$ refines to $T'$ guarantees that the
sequential conjunction $(S,T)$ refines to $(S',T')$.
Monotonicity holds for all the operators and both quantifiers in the
wide-spectrum language.
%; the proofs appear in \refappendix{app-monotonic}.
{\ReftLaw Monotonicity  of parallel conjunction \label{mono:para}}
\[          
    \Rule{ S \refsto S';\ T \refsto T'}
         { S \land T \refsto S' \land T' }
\]          

\reflaw{dist:seq:disj:rc} may be used to distribute a sequential
conjunction through a disjunction.
%Other distribution and associativity laws
%are presented in \refappendix{dist:assoc}.
{\ReftLaw Distribute sequential \label{dist:seq:disj:rc}}
\[
    S, (T \lor U) \refeq (S, T) \lor (S, U)
\]


We may unfold a non-recursive parameterised command.
%For the purposes of this discussion,
Recall that 
the expression $\replace{S}{V}{T}$ represents the command $S$ with all
occurrences of free variable $V$ replaced with term $T$.
%We express a command $S$ with free variables $X$ as $\pfree{S}{X}$.
{\ReftLaw Parameterise \label{parameterise:rc}}
\[
    \replace{S}{V}{T} \refeq (V \prm S)(T)
\]


\COMMENT{
We may also unfold a call on a recursive block.  Inside the block is
a program $\C(p)$, which is a command with free variable $V$ and recursive
calls on
procedure $p$.  If the block is applied to actual
parameter $T$, it is equivalent to $\replace{\C(p')}{V}{T}$,
where $p'$ is the original
recursion block.
{\ReftLaw Unfold recursion \label{rec:unfold:rc}}
\[
    (\re p @ V \prm \C(p) \er)(T) \refeq 
        \replace{\C(\re p @ V \prm \C(p) \er)}{V}{T}
\]
\reflaw{rec:unfold:rc} may be reformulated as follows.
\[
    pc(T) \refeq \replace{\C(pc)}{V}{T} \\
    \mbox{where}\ pc \sdef \re p @ V \prm \C(p) \er
\]
For example, given the following definition,
\[
    nats \sdef \rec(nat, {\pcmd(V, {\Spec{V = 0} \lor 
        (\exists Y @ \Spec{V = s(Y)}, nat(Y))})})
\]
a procedure call $nats(T)$ refines to
\[
    \Spec{T = 0} \lor (\exists Y @ \Spec{T = s(Y)}, nats(Y))
\]
}




\subsection{Example refinement}

We present an example refinement using some of the laws presented above.  We
implicitly use monotonicity so that the refinement of a subprogram refines the
program as a whole.
\begin{derivation}
    \step{\Ass{X = 5}, \Spec{Y = X+10 \lor Y = X + 20}}
    \trans{\refeq}{\reflaw{lift:disj}}
    \step{\Ass{X = 5}, (\Spec{Y = X+10} \lor \Spec{Y = X + 20})}
    \trans{\refeq}{\reflaw{dist:seq:disj:rc}}
    \step{(\Ass{X = 5}, \Spec{Y = X+10}) \lor (\Ass{X = 5}, \Spec{Y = X + 20})}
    \trans{\refsto}{\reflaw{ctx:ass:spec:refsto:rc} \crosstwo}
    \step{(\Ass{X = 5}, \Spec{Y = 15}) \lor (\Ass{X = 5}, \Spec{Y = 25})}
    \trans{\refsto}{\reflaw{remove:ass} \crosstwo}
    \step{\Spec{Y = 15} \lor \Spec{Y = 25}}
\end{derivation}
        
We leave the refinement at this point, since it is a disjunction of primitive
specification statements.  The proof obligation for
the second last step, in the two applications of \reflaw{ctx:ass:spec:refsto:rc},       
was:    
\[  
    X = 5 \entails (Y = X+10 \iff Y = 15) \land \\
    X = 5 \entails (Y = X+20 \iff Y = 25) \\
\]  





==> setlist.tex <==
\section{Set/List module example}
\label{setlist:ax}

\begin{figure}
\[
  \Module\ Set \\
	\t1 \mtype\ \setnat == \fset \nat \\
\also
	\t1 init (S':\ \setnat_o) \\
	\t1 add (E: \nat, S:\ \setnat_i, S':\ \setnat_o) \\
	\t1 mem (E: \nat, S:\ \setnat_i) \\
	\t1 union (S_1: \setnat_i, S_2:\ \setnat_i, S':\ \setnat_o) \\
\also
	\t1 init (S') \sdef \Spec{S' = \es} \\
	\t1 add (E, S, S') \sdef \Ass{S \in \setnat \land E \in \nat 
			\land  E \notin S}, 
		\Spec{ S' = S \union \{E\}}\\
	\t1 mem (E, S) \sdef \Ass{S \in \setnat}, 
		\Spec{ E \in S} \\
	\t1 union (S_1, S_2, S') \sdef 
			 \Ass{S_1 \in \setnat \land S_2 \in \setnat}, 
			 \Spec{S' = S_1 \union S_2} \\
  \End
\]
\caption{Abstract set module \label{module:set}}
\end{figure}

\begin{equation}
\label{setlist:CI}
	CI == S = \ran L \land L \in \listnat
\end{equation}


The function `$\ran$' returns the set of elements in a list 
and $\listnat$ is the
type representing a finite list of natural numbers.  
\reffig{module:set+} gives an implementation of the set module using
the type $\listnat$.
We use the convention that the names of concrete modules and procedures
%and variables 
are superscripted with `+'. 
\begin{figure}[t]
% The complete concrete module, $Set^+$,
% that corresponds to the abstract module $Set$, is
\[
	\Module\ Set^+ \\
		\t1 \mtype\ \listnat ==
			\{L:list | \ran L \in \fset \nat\} \\
		\also
		\t1 init^+(L':\ \listnat_o) \\
		\t1 add^+(E: \nat, L: \listnat_i, L': \listnat_o) \\
		\t1 mem^+(E: \nat, L:\ \listnat_i) \\
		\t1 union^+(L_1: \listnat_i, L_2: \listnat_i, L': \listnat_o) \\
		\also
		\t1 init^+(L') \sdef \Spec{L' = \el} \\
		\t1 add^+(E,L,L') \sdef 
			\Ass{L \in \listnat \land E \in \nat \land E \notin \ran L},
			\Spec{L' = [E|L]} \\
		\t1 mem^+(E,L) \sdef \Ass{L \in \listnat}, 
			\Spec{E \in \ran L} \\
		\t1 union^+(L_1,L_2,L') \sdef 
			\Ass{L_1 \in \listnat \land L_2 \in \listnat},
			\Spec{L' = L_1\cat L_2} \\
	\End
\]
\caption{Concrete set module \label{module:set+}}
\end{figure}

\subsection{Inefficient implementation using the naive approach}
\label{dr:weak}

For example,
although $Set^+$ is intuitively an implementation of $Set$
given the chosen coupling invariant,
consider the proof of \refeqn{case1:reftrule} for $add$ and $add^+$.
\[
	(S = \ran L \land L \in \listnat \land 
				S' = \ran L' \land L' \in \listnat ) \entails \\
		\t1 (S \in \setnat \land E \in \nat \land E \notin S) \imp \\
			\t2 (L \in \listnat \land E \in \nat \land E \notin \ran L) \land \\
			\t2 (S' = S \union \{E\} \iff L' = [E|L])
\]
The equivalence on the bottom line does not hold -- it holds only in
the `$\follows$' direction.
There are many list representations for any non-empty set:
any permutation of a list that contains all the
elements of the set, possibly with some elements of the set appearing
multiple times in the list.
% for example, we could have had $E$ being appended to the end of
% $L$).
To establish an equivalence in the bottom line above,
we would need to replace $L' = [E|L]$ by $\ran L' = \{E\} \cup \ran L$.
This has the effect in the implementation of (trying to)
generate all such list representations.
However, just one representation is sufficient because 
we are not directly interested in the representations
of intermediate lists;
we are only interested in the sets they represent.

\subsection{Inefficient derivation}
\label{mr:weak}

For instance, consider deriving the list implementation of adding an
element to a set.
After simplification, the
derived concrete implementation using $S = \ran L$ as the coupling
invariant would be:
\[
	add(E, L, L') \sdef 
		\Ass{L \in \listnat \land E \in \nat \land E \notin \ran L},
		\Spec{\ran L' = \{E\} \union \ran L}
\]
It is not possible to refine this to the implementation using $L' = [E|L]$;
we require all solutions to adding an element to a list, not just the
instance where the element is added to the head of the list.

We may prove \refcond{combined} using $L' = [E|L]$ (see \cite{Thesis}),
however it is undesirable to work with such a large proof for what is
a straightforward relationship.

\subsection{Proof that $Set$ and $Set^+$ satisfy \refth{th:mod:reft}}

The full instantiation of \refcond{combined} for $add$ and $add+$ is:
\[
	S' \nfi (S \in \setnat \land E \in \nat \land E \notin S) \land \\
	L' \nfi (L \in \listnat \land E \in \nat \land E \notin \ran L) \land \\
	\also
	S = \ran L \land L \in \listnat \land S \in \setnat \land 
				E \in \nat \land E \notin S \entails \\
		\t1 L \in \listnat \land E \in \nat \land E \notin \ran L \land \\
		\t1 (S' = \{E\} \union S \imp (\exists L' @ L' = [E|L] \land
			S' = \ran L' \land L' \in \listnat)) \land \\
		\t1 (L' = [E|L] \imp (\exists S' @ S' = \{E\} \union S \land
			S' = \ran L' \land L' \in \listnat)) %\land \\
\]
This is straightforward to show by using the one-point law on the
existentially quantified variables.

Because there are no opaque inputs, and for both $init$ and $init^+$
the $ok$ condition is just
$true$, the instantiated \refcond{combined} for $init$ and $init^+$ is
the following easily validated condition.
\[
	(S' = \es \entails 
		(\exists L' @ L' = \el \land S' = \ran L' \land L' \in \listnat)) \land \\
	(L' = \el \entails 
		(\exists S' @ S' = \es \land S' = \ran L' \land L' \in \listnat)) 
	%((S = \es \land L = \el) \imp S = \ran L \land L \in \listnat)
\]

For the $mem$ procedure of the set module,
instantiating (\ref{combined:observer}) gives:
\[
	S = \ran L \land L \in \listnat \inctx \\
		\t1 \Ass{S \in \setnat}, \Spec{E \in S} \refsto
			\Ass{L \in \listnat}, \Spec{E \in \ran L} \\  
\]
We can show this holds
from \reflaw{weaken:ass} and \reflaw{equiv:specs}.

\COMMENT{
Instantiating \refcond{combined} (with \refeqn{proofob:freeOutputs} satisfied
trivially) for the $union$ procedures gives:
\[
    S_1 = \ran L_1 \land L_1 \in \listnat \land S_2 = \ran L_2 \land L_2 \in
	\listnat \land \\
	S_1 \in \setnat \land S_2 \in \setnat \entails \\
		\t1 L_1 \in \listnat \land L_2 \in \listnat \land \\
	    \t1  S' = S_1 \union S_2 \imp 
			(\exists L' @ L' = L_1 \cat L_2 \land S' = \ran L' \land L' \in
			\listnat) \land\\
	    \t1  L' = L_1 \cat L_2 \imp 
			(\exists S' @ S' = S_1 \union S_2 \land S' = \ran L' \land L' \in
			\listnat)
\]
This follows by using the one-point rule and
the definition of $\ran$.
}


We have shown that all three procedures of $Set$ and $Set^+$
are related to their counterparts via the coupling invariant $S = \ran L \land
L \in \listnat$ and \refcond{combined}.
Hence, by \refth{th:mod:reft},
a program that is in \opqf\ w.r.t. $Set$ may be refined to the
equivalent program that is in \opqf\ w.r.t. $Set^+$.
%the module $Set$ may be replaced by $Set^+$ for use in any
%program in \opqf\ w.r.t. $Set$.
%(\refdefn{pgm:form}).
%that respects \refcond{combined:nfi}.



In this example, the coupling invariant chosen, $S = \ran L \land L \in
\listnat$, allowed efficient
implementation of $add^+$ and $union^+$.  However the coupling invariant is not
strong enough to allow efficient implementation of 
a procedure $remove$, which deletes an element $E$ from the set.  
We would have to
ensure that all instances of $E$ in the list $L$ are removed.  Removing
just the first occurrence of $E$ from $L$, resulting in $L'$, 
would not ensure the coupling invariant holds for the
opaque outputs, since it would not necessarily be true that 
$\ran L' = S - \{E\}$.
%Alternatively, we could choose a concrete representation of an ordered list
%with no duplicates, 

\COMMENT{
\subsection{Instantiation of inductive proof}

To further explain the refinement
in \reffig{ind:reft}, we demonstrate how it would be
used in a particular example.  Note that this is for illustrative purposes
only; the following steps would not need to be taken if \refcond{combined} is
shown for each pair of related procedures in the two modules.

Consider the following program, which is in \opqf\ w.r.t. $Set$.
\[
    (\exists S @ init(S), (\exists S' @ add(1,S,S'), mem(X,S')))
\]
We refine this program to its concrete counterpart that uses the module $Set^+$.
We follow the proof steps outlined in \reffig{ind:reft}.
%, the obligations for which have been shown elsewhere.
In brief, we combine steps 1 and 2 to introduce the concrete initialisation and
the coupling invariant.
Then, since the coupling invariant has been established for the
opaque inputs to $add$, we may also introduce the concrete $add^+$.  This then
provides the coupling invariant for opaque inputs to $mem$; we can thus replace
it
with the concrete version $mem^+$.
We then backtrack, removing the abstract calls and
variables by combining steps 4 and 5.
We use the shorthand $CI(S,L)$ for $S = \ran L \land L \in \listnat$.

\begin{derivation}
    \step{(\exists S @ init(S), (\exists S' @ add(1,S,S'), mem(X,S')))}
    \trans{\refsto}{introduce $init^+(L) \land \Spec{CI(S,L)}$,
		combining steps 1 and 2}
    \step{(\exists S,L @ (init(S) \land init^+(L) \land CI(S,L)), }
        \step{\t1 (\exists S' @ add(1,S,S'), mem(X,S')))}
    \transbox{\refsto}{with $CI(S,L)$ in context, introduce $add^+ \land CI(S',L')$
            by combining steps 1 and 2}
    \step{(\exists S,L @ (init(S) \land init^+(L) \land CI(S,L)), }
        \step{\t1 (\exists S',L' @ (add(1,S,S') \land add^+(1,L,L') \land
		CI(S',L')), }
        \step{\t1 mem(X,S')))}
    \trans{\refsto}{we may refine the call to $mem(X,S')$ to $mem^+(X,L')$}
    \step{(\exists S,L @ (init(S) \land init^+(L) \land CI(S,L)), }
        \step{\t1 (\exists S',L' @ (add(1,S,S') \land add^+(1,L,L') \land
		CI(S',L')), }
        \step{\t1 mem^+(X,L')))}
    \trans{\refsto}{combine steps 4 and 5 to eliminate redundant $S'$}
    \step{(\exists S,L @ (init(S) \land init^+(L) \land CI(S,L)), }
        \step{\t1 (\exists L' @ add^+(1,L,L'), mem^+(X,L')))}
    \trans{\refsto}{combine steps 4 and 5 to eliminate redundant $S$}
    \step{(\exists L @ init^+(L), (\exists L' @ add^+(1,L,L'), mem^+(X,L')))}
\end{derivation}

\def \CITCL {(T,C) = (\sum L, \#L) \land (T,C) \in \calc}
\def \CITCLP {(T',C') = (\sum L', \#L') \land (T',C') \in \calc}

}


